Shortest Paths in Graphs of Convex Sets

Given a graph, the shortest-path problem requires finding a sequence of edges with minimum cumulative length that connects a source vertex to a target vertex. We consider a variant of this classical problem in which the position of each vertex in the graph is a continuous decision variable constrained in a convex set, and the length of an edge is a convex function of the position of its endpoints. Problems of this form arise naturally in many areas, from motion planning of autonomous vehicles to optimal control of hybrid systems. The price for such a wide applicability is the complexity of this problem, which is easily seen to be NP-hard. Our main contribution is a strong and lightweight mixed-integer convex formulation based on perspective operators, that makes it possible to efficiently find globally optimal paths in large graphs and in high-dimensional spaces.

==> sections/contributions.tex <==
The following list collects the main contributions of this article:
\begin{itemize}
\item
\emph{Problem statement.}
The SPP in GCS lends itself to a very simple and compact problem statement and, at the same time, it is a very versatile framework that includes as special cases many problems of practical relevance at the intersection of combinatorial and convex optimization.
\item
\emph{Mixed-integer convex formulation.}
The SPP in GCS is easily seen to be NP-hard.
For its solution we design a strong Mixed-Integer Convex Program (MICP) that can be effectively solved to global optimality via branch and bound.
%By using perspective functions (a tool from convex analysis that has seen multiple applications in mixed-integer programming~\cite{ceria1999convex,frangioni2006perspective,gunluk2010perspective,gunluk2012perspective}), this MICP extends in a very natural way the classical network-flow formulation of the SPP.
This MICP extends in a very natural way the classical network-flow formulation of the SPP, it tackles the problem in its full generality, and it allows us to reliably find shortest paths even when working with large graphs and in high-dimensional spaces.
%This formulation integrates in a novel and natural way classical results from network flows and modern tools from convex optimization.
\item
\emph{Convex relaxation of bilinear constraints.}
The main building block of our MICP is a tight and compact convex relaxation for bilinear functions defined over the Cartesian product of convex sets.
%a class of bilinear constraints that emerge naturally in our analysis.
%We will show that the SPP in GCS is naturally formulated as an optimization problem with bilinear equality constraints.
%The main technical tool we use in the design of the MICP is a  convex relaxation of these bilinearities.
%design is a tight and compact convex relaxation of bilinear functions defined over the Cartesian product of convex sets.
%The main technical tool used in the design of the MICP is a convex relaxation of a class of bilinear constraints that emerge in our analysis.
The principle behind this relaxation is the well-known Reformulation-Linearization Technique (RLT)~\cite{sherali1990hierarchy,sherali1992new}.
However, by using the language of perspective functions (a tool from convex analysis that has seen multiple applications in mixed-integer programming~\cite{ceria1999convex,frangioni2006perspective,gunluk2010perspective,gunluk2012perspective}), our analysis applies to generic convex sets and does not require to work with the explicit expressions of the constraints that define these sets.
This greatly simplifies the analysis.
\item
\emph{Control applications.}
At present, computation times are the main limitation to a widespread application of mixed-integer optimization in control of hybrid systems~\cite{naik2017embedded,stellato2018embedded,hespanhol2019structure,marcucci2020warm,bertsimas2022online}.
%For optimal control of hybrid dynamical systems~\cite{bemporad1999control}, o
Our framework leads to MICPs that can be orders of magnitude faster to solve than state-of-the-art mixed-integer formulations of these problems~\cite{moehle2015perspective,marcucci2019mixed}.
\end{itemize}
